Fully-Discretely Nonlinearly-Stable Flux Reconstruction Methods for Compressible Flows

A fully-discrete, nonlinearly-stable flux reconstruction (FD-NSFR) scheme is developed, which ensures robustness through entropy stability in both space and time for high-order flux reconstruction schemes. We extend the entropy-stable flux reconstruction semidiscretization of Cicchino et al. [1,2,3] with the relaxation Runge Kutta method to construct the FD-NSFR scheme. We focus our study on entropy-stable flux reconstruction methods, which allow a larger time step size than discontinuous Galerkin. In this work, we develop an FD-NSFR scheme that prevents temporal numerical entropy change in the broken Sobolev norm if the governing equations admit a convex entropy function that can be expressed in inner-product form. For governing equations with a general convex numerical entropy function, temporal entropy change in the physical $L_2$ norm is prevented. As a result, for general convex numerical entropy, the FD-NSFR scheme achieves fully-discrete entropy stability only when the DG correction function is employed. We use entropy-conserving and entropy-stable test cases for the Burgers', Euler, and Navier-Stokes equations to demonstrate that the FD-NSFR scheme prevents temporal numerical entropy change. The FD-NSFR scheme therefore allows for a larger time step size while maintaining the robustness offered by entropy-stable schemes. We find that the FD-NSFR scheme is able to recover both integrated quantities and solution contours at a higher target time-step size than the semi-discretely entropy-stable scheme, suggesting a robustness advantage for low-Mach turbulence simulations.

==> Euler-NS/old/root_rrk_implementation.tex <==
\subsection{Relaxation Runge-Kutta for General Convex Quantities} \label{sec:RRK-root}


% \textit{Possible modified outline.}
% \begin{itemize}
%     %\item Present root-finding equation referencing Ranocha; Eq. \ref{eq:root-implementation}.
%     \item We want to extend RRK to FR, where stability is in M+K norm. Therefore, we want to solve $ \eta_{FR}(u^{n+\gamma}) - \eta_{FR} (u^n) -\gamma^n \Delta t \sum_{i=1}^s b_i \textbf{v}^{(i),T} (\mathcal{M}+\mathcal{K}) \frac{d\textbf{u}^{(i)}}{dt} = 0$.
%     \item Problem with calculating $\eta_{FR}$: we don't know how to integrate in a form like $\int_{\Omega_m} S(\bm{u}_m) + \frac{\partial^p}{\partial \xi^p} S(\bm{u}_m) d\Omega_m$. (proof?)
    
%     \item Thm: Solving in \ref{eq:root-implementation} ensures that $\Delta \eta_{FR}$ will follow $e_{M+K}$.
%     \begin{itemize}
%         \item Suppose that we are concerned with ensuring stability in $e_{M+K}$. Define the change in entropy over a time step as $\Delta \eta_{FR} = e_{M+K}$.
%         \item Then, $\Delta \eta_{FR} = e_{M}+e_{K} = \eta(u^{n+\gamma}) - \eta(u^{n}) + e_K$.
%     \end{itemize}
% \end{itemize}

% \textit{Writing out the logic we are using when calculating $\Delta \eta_{FR}$.}
% \begin{enumerate}
%     \item We want information about the evolution of entropy in the $M+K$ norm, therefore we are interested in tracking $\gamma e_{M+K}$, which is an estimate of the entropy change over the time step to the order of the RK scheme in the $M+K$ norm. Any entropy change other than $\gamma e_{M+K}$ is assumed to be due to the RK temporal integration and therefore is undesirable for an entropy-stable scheme.
%     \item We cannot directly calculate $\eta_{FR} = \int_{\Omega_m}( S(\bm{u}_m) + \frac{\partial^p}{\partial \xi^p} S(\bm{u}_m) )d\Omega_m$. ** with caveat that it may not look exactly as I
%     ve written it
%     \item We suppose that the entropy change over a time step can be expressed as a FR-corrected entropy change of the form $\Delta \eta_{FR} = \eta(u^{n+\gamma})-\eta(u^n) + C_{FR}$. $C_{FR}$ is a correction which accounts for $\int_{\Omega} \frac{\partial^p}{\partial \xi^p}S(u^{n+\gamma}) d \Omega - \int_{\Omega} \frac{\partial^p}{\partial \xi^p}S(u^{n}) d \Omega$. The FR-corrected entropy change will follow the entropy change estimate $\Delta \eta_{FR} = \gamma e_{M+K}$.
%     \item Since we define $\gamma$ such that $\eta(u^{n+\gamma}) - \eta(u^n) = \gamma e_M$, we have $C_{FR} = \gamma e_{K}$.
%     \begin{itemize}
%         \item Issue with this step: We know that $C_{FR}$ is a function of $\gamma$ because it's a placeholder for a nonlinear function of $u$. It's puzzling that it would turn out to just be in the form $\gamma [constant]$; how would scaling a constant by $\gamma$ account for a nonlinear function?
%     \end{itemize}
%     \item not generating temporal entropy ** in the M norm **.
% \end{enumerate}


The root equation (\ref{eq:RRK_explicit}) as presented in section \ref{sec:RRK-overview} can be solved analytically when energy is the numerical entropy variable~\cite{ketcheson2019relaxation}. 
However, the Euler and Navier-Stokes equations do not have a numerical entropy function that can be written in an inner-product form. 
Rather, it is a convex nonlinear function.
In such cases, we adopt the approach of~\cite{ranocha2020relaxation}.
If the numerical entropy is a general convex function, we implement eq.~(\ref{eq:rrk-root}) as a root-finding problem
\begin{equation}
    r(\gamma^n)=\sum_{m=1}^N \int_{\Omega^m} S(\mathbf{u}_m^{n+\gamma}) d\Omega^m - \sum_{m=1}^N \int_{\Omega^m} S(\mathbf{u}_m^{n}) d\Omega^m - \gamma^n \Delta t \sum_{i=1}^s b_i \langle \textbf{v}^{(i)}, \frac{d\textbf{u}^{(i)}}{dt} \rangle_{L^2},
    \label{eq:root-implementation}
\end{equation}
\noindent where the total entropy over the domain is $\eta(\mathbf{u}) =\int_{\Omega} S(\mathbf{u})\; d\Omega$. To calculate the integrated numerical entropy in the first two terms of the left-hand side of Eq.~(\ref{eq:root-implementation}), we integrate the numerical entropy function $S(\mathbf{u})$ over the solution nodes of the $N$ elements in the domain.
The resulting $\eta$ is in the physical $L^2$ norm. 
In the case of a general nonlinear numerical entropy function $S(\mathbf{u})$, we cannot simply modify the norm to the broken Sobolev $W_2^p$ norm as we did for the inner-product numerical entropy functions in Section \ref{sec:RRK-implementation-scalar}.

To calculate the entropy change estimate, we use an inner product between the entropy and conservative variables in the $L^2$ norm, i.e.,
\begin{equation}
    \langle \mathbf{v}^{(i)}, \frac{d\mathbf{u}^{(i)}}{dt} \rangle_{L^2} = \mathbf{v}^T \mathcal{M} \frac{d\mathbf{u}^{(i)}}{dt}
\end{equation}
\noindent which uses the unmodified mass matrix. 
The $L^2$ norm is employed, to ensure consistency with the integrated numerical entropy terms.

The implementation as described by Eq. (\ref{eq:root-implementation}) is similar to that proposed by Ranocha \textit{et al.}~\cite{ranocha2020relaxation}, and the proofs therein apply immediately when the $c_{DG}$ correction parameter is applied and the discretization is stable in the $L^2$ norm. 
When nonzero correction parameters are used, one is still restricted to the implementation in Eq. (\ref{eq:root-implementation}).
Therefore, we solve for $\gamma^n$ in the $L^2$ norm for any $c$, and present discrete results which demonstrate the validity of this strategy.

\begin{remark}
    Entropy stability proofs for the NSFR scheme are in the $W_2^p$ norm~\cite{cicchino2021new,cicchino2022nonlinearly,cicchino2022provably,cicchino2023discretely}.
    In section~\ref{sec:RRK-implementation-scalar}, we simply calculated the integrated numerical entropy and entropy change estimate consistently in the $W_2^P$ norm through the definition of the inner product.
    However, this strategy could not be directly applied to general convex numerical entropy functions because it is no longer trivial to evaluate the integrated numerical entropy in the $W_2^p$ norm.
\end{remark}

We follow the proofs of Ranocha \textit{et al.}~\cite{ranocha2020relaxation} and discretely demonstrate that they are upheld for the range of the correction parameter $c$ based on the original ESFR scheme~\cite{castonguay2012high,zwanenburg2016equivalence}, which we define as $c_{DG} \leq c \leq c_+$. 
For the $L^2$-norm case, Ranocha \textit{et al.}~\cite{ranocha2020relaxation} established existence and accuracy of the method by showing that the root function is convex with a root at $0$ and another close to $1$. 
We use the inviscid Taylor-Green vortex test case, which will be introduced in section \ref{sec:inv-tgv}, as an entropy-conserving Euler test case.
We demonstrate discretely that the root function is convex with a root close to $1$ in Figure~\ref{fig:RRK-root-Euler} (a). This is true for both $c_{DG}$ and $c_+$. Moreover, the choice of $c$ does not appear to change the form of the root equation, reflected in the similar shape of the root equation for both correction parameters shown.

To confirm the convexity of the root function, we calculate the slope of the root equation at every time step using finite difference. 
The slope is strictly negative at $\gamma=0$ and strictly positive at $\gamma=1$ for all time using either correction parameter as observed in Fig.~\ref{fig:RRK-root-Euler}(top and middle).
This is true regardless of the sign and magnitude of the $L^2$-norm entropy change estimate (as seen in the bottom plot of Figure \ref{fig:RRK-root-Euler}). 
Furthermore, we will provide confirmation of the convergence orders in subsequent sections for both $c$ parameters in a variety of test cases.

\begin{figure}[h!]
\centering
\begin{subfigure}[t]{0.48\textwidth}
    \centering
        \includegraphics[height = 5 in]{Figures/RRK_root_function.pdf}
    \caption{The root function plotted as a function of $\gamma$ for the inviscid TGV test case for $c_{DG}$ (top) and $c_+$ (bottom). }
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.48\textwidth}
    \centering
    \includegraphics[height = 5 in]{Figures/RRK_root_prime.pdf}
    \caption{The slope of the root function  at $\gamma=0$ (top), at $\gamma=1$ (middle), and the entropy change estimate $e_{L^2}\coloneqq \Delta t \sum_{i=1}^s b_i \langle \bar{\textbf{v}}^{(i)}, \frac{d\bar{\textbf{u}}^{(i)}}{dt} \rangle_{L^2}$(bottom), plotted over the simulation time. Even in the low-$t$ region, $r^\prime(1)>0$ and $r^\prime(0)<0$.}
\end{subfigure}
    \caption{The root function for $c_{DG}$ and for $c_+$, plotted per the implementation in Eq.~(\ref{eq:root-implementation}). The test case is as described in Section \ref{sec:inv-tgv}, using the largest stable CFL, i.e. $CFL=0.48$ for the $c_{DG}$ version, and $CFL = 0.54$ for the $c_+$ version.}
    \label{fig:RRK-root-Euler}
\end{figure}

\begin{remark}
    By solving the root equation in the $L^2$,  we find $\gamma^n$ such that temporal entropy generation \textit{in the $L^2$ norm} is accounted for. 
    It is assumed that the same $\gamma$ would result if we were to solve entirely in the $W_2^P$.
    When using a nonzero correction parameter, we filter the highest mode enough to add stability, but not so much that we lose an order. The filtering therefore has only a subtle impact on the solution as a whole. Our numerical results, which show conservation at machine precision, support that solving in the $L^2$ norm is sufficient to also account for the difference from the $W_2^p$ norm.
\end{remark}

While we have demonstrated that filtering with a nonzero $c$ parameter does not greatly change the properties of the root function, we also require a means of confirming that numerical entropy is conserved or dissipated in the appropriate $W_2^p$ norm.
We propose the following definition which corrects the $L^2$ numerical entropy change such that we can verify that numerical entropy is indeed conserved or dissipated.

\begin{definition}
In the case of NSFR schemes, which are entropy-stable in the broken Sobolev norm, we verify conservation or stability in the broken Sobolev norm by reporting $\eta_{FR}^n$, which we call the ``FR-corrected entropy change", \begin{equation}
    \Delta \eta_{FR}^n=\eta(\mathbf{u}^{n+\gamma}) - \eta(\mathbf{u}^{n}) + \gamma^n \Delta t \sum_{i=1}^s b_i \textbf{v}^T  \mathcal{K} \frac{d\textbf{u}}{dt}.
    \label{eq:eta_FR}
\end{equation}
\end{definition}

To justify the definition of $\eta_{FR}$, we note that the root equation (\ref{eq:root-implementation}) can be expressed as
\begin{equation}
    r(\gamma^n)=\Delta \eta_{FR}^n -  \gamma^n \Delta t \sum_{i=1}^s b_i \langle \mathbf{v}^{(i)}, \frac{d\textbf{u}^{(i)}}{dt} \rangle_{W_2^P}
    \label{eq:root-M+K}
\end{equation}
\noindent by referring to the definition of an inner product in each norm.

\begin{remark}
    In the following sections, we demonstrate that this assumption is suitable for $c$ parameters between $c_{DG}$ and $c_+$ by showing conservation to machine precision.
    Furthermore, we report the convergence of $\gamma^n$ toward $1$, and see that we maintain an order of $p-1$ for any $c$ tested.
\end{remark}

% \begin{equation}
%     e_{\mathcal{M} + \mathcal{K}} := \Delta t \sum_{i=1}^s b_i \textbf{v}^T (\mathcal{M}+ \mathcal{K}) \frac{d\textbf{u}}{dt}  \leq 0,
% \end{equation}
% \noindent where shorthand is used for simpler notation.

% Due to linearity, we can separate the DG and FR contributions of entropy:
% \begin{equation}
%     e_{\mathcal{M} + \mathcal{K}} = e_{\mathcal{M}} + e_{\mathcal{K}}
% \end{equation}
% \noindent where $e_{\mathcal{M}}$ and $e_{\mathcal{K}}$ are defined alike $e_{\mathcal{M}+\mathcal{K}}$.

% Therefore, we can add and subtract $e_{\mathcal{K}}$ to express eq.~(\ref{eq:root-implementation}) as 
% \begin{equation}
%     r(\gamma^n)=\eta(\bm{u}^{n+\gamma}) -\eta(\bm{u}^n) +  \gamma^n  e_{\mathcal{K}} - \gamma^n e_{\mathcal{M} + \mathcal{K}}.
%     \label{eq:proof-intermediate}
% \end{equation}

% We interpret the first terms of eq.~(\ref{eq:proof-intermediate}) as an FR-corrected entropy change, which will follow the higher-order entropy change estimate $ e_{\mathcal{M} + \mathcal{K}}$ of the NSFR scheme. We define the FR-corrected entropy change as 
% \begin{equation}
%     \Delta \eta_{FR}=\eta(\bm{u}^{n+\gamma}) - \eta(\bm{u}^n) +  \gamma^n e_{\mathcal{K}},
%     \label{eq:eta_FR}
% \end{equation}
% \noindent which will evolve according to the entropy estimate in the broken Sobolev norm,
% \begin{equation}
%     r(\gamma^n)=\Delta \eta_{FR} - \gamma^n \Delta t \sum_{i=1}^s b_i \langle \textbf{v}^{(i)}, \frac{d\textbf{u}^{(i)}}{dt} \rangle_{W_2^P}.
%     \label{eq:root-M+K}
% \end{equation}

% Therefore, we may use eq.~(\ref{eq:root-implementation}) to find the relaxation parameter $\gamma^n$ which ensures entropy stability. Furthermore, we can report FR-corrected entropy change $\Delta \eta_{FR}$ to verify that we achieve the correct entropy evolution.

% We use Equation~(\ref{eq:root-M+K}) to show that the convergence properties of RRK are maintained.

% \subsubsection{Existence of a Solution and Accuracy}

% % \textcolor{blue}{}

% % \subsubsection{Accuracy of Relaxation Runge-Kutta for General Convex Quantities}
% Refer the reader to Thm. 2.11 in Ranocha since we are using the same root-finding function.

\subsubsection{Implementation of the root-solving method}

We choose to use the secant method in order to numerically find the root of Eq.~(\ref{eq:root-implementation}), aligning with the recommendations of Al Jahdali \textit{et al.}~\cite{aljahdali2022on} and Rogowski \textit{et al.} ~\cite{rogowski2022performance}. In order to improve the robustness of the root-finding problem, we have implemented Algorithm~\ref{alg:root} to find $\gamma^n$. We found the algorithm to be robust. The bisection method was rarely used in the numerical experiments and is included as a safeguard to prevent crashes.

\begin{algorithm}
    \caption{Root-finding algorithm.}
    \label{alg:root}
    \begin{algorithmic}
    \State $tolerance \gets 5E-10; \ \ iterationLimit \gets 100$
    \State $\gamma^k \gets \gamma^n + 1E-5$ and $\gamma^{k-1} \gets \gamma^n - 1E-5$
    \State $r_k \gets $ \Call{root eq.}{$\gamma_k$}$;\ \  r_{k-1} \gets $ \Call{root eq.}{$\gamma_{k-1}$}
    \State residual $\gets 1$; $iterationCounter \gets 0$
    \While{$residual > tolerance$ and $iterationCounter < iterationLimit$} \Comment{Secant method loop}
        \State $\gamma_{k+1} \gets \gamma_k - r_k \frac{\gamma_k - \gamma_{k-1}}{r_k-r_{k-1}}$ \Comment{Secant method}
        \If{$\gamma^{k+1} < 0.5$ or $\gamma^{k+1} > 1.5$ or $\gamma^{k+1}$ is NaN}
            \State $\gamma^k = 1 + 10^{-5}$ and $\gamma^{k-1} = 1 - 10^{-5}$ \Comment{reinitialize from $1$ if the current value is far from $1$}
        \EndIf
        \State $\gamma_{k-1} \gets \gamma_k;\ \ \gamma_k \gets \gamma_{k+1}$
        \State $r_{k-1} \gets r_k;\ \ r_k \gets$ \Call{root eq.}{$\gamma_k$}
        \State $residual \gets |\gamma_k - \gamma_{k-1}|$
        \State $iterationCounter++$
    \EndWhile   
    \If{$iterationCounter == iterationLimit$ and $residual > tolerance$} \Comment{Bisection method loop}
    \State $\gamma^k \gets \gamma^n + 0.1$ and $\gamma^{k-1} \gets \gamma^n - 0.1$, and reset $iterationCounter = 0$.
    \While{$residual > tolerance$ and $iterationCounter < iterationLimit$}
        \IIf{there is no root in the interval} increase interval size by 0.1\EndIIf
        \State update $\gamma^{k+1}$ with Bisection method
        \State $\gamma^k \gets \gamma^{k+1}$ and $\gamma^{k-1} \gets \gamma^k$ and $residual = |\gamma^{k+1} - \gamma^k|$
        \State $iterationCounter++$
    \EndWhile
    \EndIf
    \IIf{$residual > tolerance$} abort \EndIIf
    \State $\gamma^{n+1} \gets \gamma^k$
    \end{algorithmic}

\end{algorithm}

